Discrete field theory: symmetries and conservation laws

We present a general algorithm constructing a discretization of a classical field theory from a Lagrangian. We prove a new discrete Noether theorem relating symmetries to conservation laws and an energy conservation theorem not based on any symmetry. This gives exact conservation laws for several theories, e.g., lattice electrodynamics and gauge theory. In particular, we construct a conserved discrete energy-momentum tensor, approximating the continuum one at least for free fields. The theory is stated in topological terms, such as coboundary and products of cochains.

==> networks.tex <==
\small
\ctikzset{bipoles/length=.8cm}
\begin{circuitikz}[scale=1.2]
\draw[color=brown]
(0,0) to[R, *-*] (1,0)
      to[R, *-*] (2,0)
      to[R, *-*] (3,0)
      to[short, *-] (3,0.5)
      to[american current source] (0,0.5)
      %to[battery, l=$1\mathrm{V}$] (0,0.5)
      to[short, -*] (0,0)

{[anchor=south west] (0,0) node {$+$}}
{[anchor=north](0,0) node {0} (1,0) node {1} (2,0) node {2} }
{[anchor=north] (3,0) node {3}}
{[anchor=south east] (3,0) node {$-$}}
;\end{circuitikz}


==> square-l.tex <==
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]\clip(-7.18,-5.64) rectangle (2.8,1.14);\draw [line width=2pt] (-7,0)-- (-7,1);\draw [line width=2pt,dash pattern=on 1pt off 1pt] (-7,0)-- (-6,0);\draw [line width=2pt,dash pattern=on 1pt off 1pt] (-6,1)-- (-7,1);\draw [line width=2pt,dash pattern=on 1pt off 1pt] (-6,0)-- (-6,1);\end{tikzpicture}
